Developers Insight On Manifest v3 Privacy and Security Webextensions

Webextensions can improve web browser privacy, security, and user experience. The APIs offered by the browser to webextensions affect possible functionality. Currently, Chrome transitions to a modified set of APIs called Manifest v3. This paper studies the challenges and opportunities of Manifest v3 with an in-depth structured qualitative research. Even though some projects observed positive effects, a majority expresses concerns over limited benefits to users, removal of crucial APIs, or the need to find workarounds. Our findings indicate that the transition affects different types of webextensions differently; some can migrate without losing functionality, while other projects remove functionality or decline to update. The respondents identified several critical missing APIs, including reliable APIs to inject content scripts, APIs for storing confidential content, and others.

==> Makefile <==
# Encoding: utf-8
# Libor Polčák

# Bibliography file
BIBLIO = literature.bib

# TeX files
TEX_FILES = main.tex \
			$(BIBLIO)

FIGURES = $(shell grep '\\includegraphics' *.tex | sed "s/.*{//" | sed "s/}//" | grep -v '\.png' | sed '/\.pdf$$/! { s/$$/.pdf/ }' | sort | uniq | tr "\n" " ")


LATEX = pdflatex
BIBTEX = bibtex
LATEX_FLAGS   =
BIBTEX_FLAGS  =

all: pdf

pdf: main

main: main.pdf

main.pdf: main.tex $(TEX_FILES) $(FIGURES)
	$(LATEX) $(LATEX_FLAGS) $(basename $<)
	$(BIBTEX) $(BIBTEX_FLAGS) $(basename $<)
	$(LATEX) $(LATEX_FLAGS) $(basename $<)
	$(LATEX) $(LATEX_FLAGS) $(basename $<)

plain: main.txt

%.txt: %.tex ${TEX_FILES}
	detex $< | awk '/./ {printf("%s ", $$0); odst=1} /^$$/ {if (odst == 1) {printf "\n\n"; odst=0}} END {printf "\n"}' | sed "s/ \+/ /g" | sed "s/ $$//" | sed "s/ ,/,/g" | sed "s/ \././g" > $@

fig/%-svg.pdf: fig/%.svg
	inkscape $< --export-type=pdf --export-filename=$@

fig/%-dot.pdf: fig/%.dot
	dot -Tpdf -Gmargin=0 -o $@ $<

fig/%-circo.pdf: fig/%.dot
	circo -Tpdf -Gmargin=0 -o $@ $<

fig/%-msc.svg: fig/%.msc
	mscgen -T svg -i $< -o $@

fig/%-msc.pdf: fig/%-msc.svg
	inkscape $< --export-pdf $@


fig/%-simpleplot.pdf: fig/%.gp
	gnuplot < $<

fig/%-plot.pdf: fig/%.gp fig/%*.data
	gnuplot < $<

clean:
	rm -f *.dvi *.log  *.aux *.blg *.ist *.nlg *.nls *.nlo *.bbl

cleanall: clean
	rm -f *.dvi *.log *.aux *.tex.backup *.sty.backup
	rm -f *.blg *.bbl *.toc *.out $(NAME).tar.gz
	rm -f *.pdf *.ps

printfilenames:
	@echo "Tex:" "$(TEX_FILES)"
	@echo "Figures:" "$(FIGURES)"

arxiv.zip: $(TEX_FILES) $(FIGURES) orcid-eps-converted-to.pdf main.bbl SCITEPRESS.sty orcid-eps-converted-to.pdf Makefile
	zip arxiv.zip $^ $(shell find ./include/ | sed -e "s/^/'/" -e "s/$$/'/")


==> include/4a <==
\begin{table}[h]
  \caption{Are participating webextensions affected by Manifest change?}
  \label{tab:4a}
  \centering
  \begin{tabular}{lr}
Response & Webextensions count\\
    \hline
Affected & 22\\
Not affected & 2\\
Likely not affected & 1\\
Not sure how affected & 4\\
Uses Mv3 from start & 1\\
Project inactive & 1\\
\end{tabular}
\end{table}

